Balanced Energy Regularization Loss for Out-of-distribution Detection

In the field of out-of-distribution (OOD) detection, a previous method that use auxiliary data as OOD data has shown promising performance. However, the method provides an equal loss to all auxiliary data to differentiate them from inliers. However, based on our observation, in various tasks, there is a general imbalance in the distribution of the auxiliary OOD data across classes. We propose a balanced energy regularization loss that is simple but generally effective for a variety of tasks. Our balanced energy regularization loss utilizes class-wise different prior probabilities for auxiliary data to address the class imbalance in OOD data. The main concept is to regularize auxiliary samples from majority classes, more heavily than those from minority classes. Our approach performs better for OOD detection in semantic segmentation, long-tailed image classification, and image classification than the prior energy regularization loss. Furthermore, our approach achieves state-of-the-art performance in two tasks: OOD detection in semantic segmentation and long-tailed image classification. Code is available at https://github.com/hyunjunChhoi/Balanced_Energy.

==> alpha_exp_merge.tex <==
\begin{table}[t!]
\captionsetup{font=footnotesize}
\caption{ Evaluation result on CIFAR using ResNet18; average (over 6 datasets) OOD detection performance (AUROC,AP, FPR) and classification accuracy (ACC) (a): Result on CIFAR10 (b): Result on CIFAR100}
\vspace{-0.2cm}
\begin{subtable}{0.25\linewidth}
\centering
\tiny
\caption{}
\label{balanced_cifar10}
\begin{tabular}{cccccccc}
\hline
\multicolumn{8}{c}{Average AUROC} \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{Gamma}} &
  \multicolumn{7}{c}{beta} \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{0.0025} &
  \multicolumn{1}{c|}{0.01} &
  \multicolumn{1}{c|}{0.025} &
  \multicolumn{1}{c|}{0.05} &
  \multicolumn{1}{c|}{0.1} &
  \multicolumn{1}{c|}{0.25} &
  0.5 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  \multicolumn{7}{c}{alpha} \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{0.5} &
  \multicolumn{1}{c|}{2} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{10} &
  \multicolumn{1}{c|}{20} &
  \multicolumn{1}{c|}{50} &
  100 \\ \hline
\multicolumn{1}{c|}{0.1} &
  \multicolumn{1}{c|}{91.92} &
  \multicolumn{1}{c|}{91.93} &
  \multicolumn{1}{c|}{91.98} &
  \multicolumn{1}{c|}{92.01} &
  \multicolumn{1}{c|}{92.12} &
  \multicolumn{1}{c|}{92.02} &
  91.52 \\ \hline
\multicolumn{1}{c|}{0.25} &
  \multicolumn{1}{c|}{91.96} &
  \multicolumn{1}{c|}{92.00} &
  \multicolumn{1}{c|}{92.07} &
  \multicolumn{1}{c|}{92.16} &
  \multicolumn{1}{c|}{92.28} &
  \multicolumn{1}{c|}{92.42} &
  91.69 \\ \hline
\multicolumn{1}{c|}{0.5} &
  \multicolumn{1}{c|}{92.17} &
  \multicolumn{1}{c|}{92.20} &
  \multicolumn{1}{c|}{92.29} &
  \multicolumn{1}{c|}{92.44} &
  \multicolumn{1}{c|}{92.55} &
  \multicolumn{1}{c|}{92.11} &
  91.85 \\ \hline
\multicolumn{1}{c|}{0.75} &
  \multicolumn{1}{c|}{92.34} &
  \multicolumn{1}{c|}{92.39} &
  \multicolumn{1}{c|}{92.48} &
  \multicolumn{1}{c|}{\textbf{92.56}} &
  \multicolumn{1}{c|}{92.50} &
  \multicolumn{1}{c|}{92.00} &
  91.82 \\ \hline
\multicolumn{1}{c|}{1} &
  \multicolumn{1}{c|}{92.41} &
  \multicolumn{1}{c|}{92.47} &
  \multicolumn{1}{c|}{92.52} &
  \multicolumn{1}{c|}{92.45} &
  \multicolumn{1}{c|}{92.44} &
  \multicolumn{1}{c|}{91.91} &
  91.79 \\ \hline
\multicolumn{1}{c|}{1.25} &
  \multicolumn{1}{c|}{92.39} &
  \multicolumn{1}{c|}{92.41} &
  \multicolumn{1}{c|}{92.37} &
  \multicolumn{1}{c|}{92.33} &
  \multicolumn{1}{c|}{92.27} &
  \multicolumn{1}{c|}{91.94} &
  91.61 \\ \hline
\end{tabular}
\end{subtable}



\begin{subtable}{0.25\linewidth}
%\vspace{0.1cm}
\caption{}
\centering
\tiny
\begin{tabular}{cccccccc}
\hline
\multicolumn{8}{c}{Average ACC(accuracy)} \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{Gamma}} &
  \multicolumn{7}{c}{beta} \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{0.0025} &
  \multicolumn{1}{c|}{0.01} &
  \multicolumn{1}{c|}{0.025} &
  \multicolumn{1}{c|}{0.05} &
  \multicolumn{1}{c|}{0.1} &
  \multicolumn{1}{c|}{0.25} &
  0.5 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  \multicolumn{7}{c}{alpha} \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{0.5} &
  \multicolumn{1}{c|}{2} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{10} &
  \multicolumn{1}{c|}{20} &
  \multicolumn{1}{c|}{50} &
  100 \\ \hline
\multicolumn{1}{c|}{0.1} &
  \multicolumn{1}{c|}{74.53} &
  \multicolumn{1}{c|}{74.60} &
  \multicolumn{1}{c|}{74.84} &
  \multicolumn{1}{c|}{75.03} &
  \multicolumn{1}{c|}{75.45} &
  \multicolumn{1}{c|}{73.71} &
  70.18 \\ \hline
\multicolumn{1}{c|}{0.25} &
  \multicolumn{1}{c|}{74.57} &
  \multicolumn{1}{c|}{74.64} &
  \multicolumn{1}{c|}{74.86} &
  \multicolumn{1}{c|}{75.23} &
  \multicolumn{1}{c|}{75.95} &
  \multicolumn{1}{c|}{76.13} &
  63.15 \\ \hline
\multicolumn{1}{c|}{0.5} &
  \multicolumn{1}{c|}{75.15} &
  \multicolumn{1}{c|}{75.23} &
  \multicolumn{1}{c|}{75.61} &
  \multicolumn{1}{c|}{75.92} &
  \multicolumn{1}{c|}{\textbf{76.60}} &
  \multicolumn{1}{c|}{68.03} &
  59.78 \\ \hline
\multicolumn{1}{c|}{0.75} &
  \multicolumn{1}{c|}{75.88} &
  \multicolumn{1}{c|}{75.87} &
  \multicolumn{1}{c|}{76.29} &
  \multicolumn{1}{c|}{76.22} &
  \multicolumn{1}{c|}{74.87} &
  \multicolumn{1}{c|}{65.64} &
  56.92 \\ \hline
\multicolumn{1}{c|}{1} &
  \multicolumn{1}{c|}{76.15} &
  \multicolumn{1}{c|}{75.92} &
  \multicolumn{1}{c|}{75.98} &
  \multicolumn{1}{c|}{74.85} &
  \multicolumn{1}{c|}{72.40} &
  \multicolumn{1}{c|}{62.86} &
  54.66 \\ \hline
\multicolumn{1}{c|}{1.25} &
  \multicolumn{1}{c|}{75.94} &
  \multicolumn{1}{c|}{75.66} &
  \multicolumn{1}{c|}{74.61} &
  \multicolumn{1}{c|}{72.38} &
  \multicolumn{1}{c|}{69.96} &
  \multicolumn{1}{c|}{60.85} &
  52.43 \\ \hline
\end{tabular}
\label{balanced_cifar100}
\end{subtable}
\end{table}


==> cls_cifar100_balanced_validation_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\scriptsize
\captionsetup{font=footnotesize}
\caption{Comparison result with other methods on CIFAR100 using ResNet18 : average (over 6 datasets) OOD detection performance (AUROC,AP, FPR) and classification accuracy (ACC)}
\label{table_cifar100_summary}
\begin{tabular}{c|c|c|c|c|c}
\hline
Dataset                  & Method          & AUC            & AP             & FPR            & ACC            \\ \hline
\multirow{5}{*}{Average} & MSP~\cite{hendrycks2016baseline}(ST)        & 76.14          & 71.29          & 62.78          & 75.70          \\
                         & Energy~\cite{liu2020energy}(ST)     & 79.78          & 73.31          & 57.59          & 75.70          \\
                         & OE~\cite{hendrycks2018deep}(tune)       & 82.76          & 78.32          & 53.50          & 79.85          \\
                         & EnergyOE~\cite{liu2020energy}(tune) & 91.42          & 88.30          & 33.29          & \textbf{80.79} \\ \cline{2-6} 
                         &  \textbf{Ours}            & \textbf{91.53} & \textbf{88.32} & \textbf{32.65} & 80.58          \\ \hline
\end{tabular}
\end{table}

==> cls_cifar100_gamma_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\centering
\footnotesize
\caption{Evaluation result on CIFAR100-LT in long-tailed image classification task depending on hyperparameter $\gamma$ : OOD detection performance(AUROC,AP,FPR)
and accuracy(ACC) with model ResNet18; Mean over six random runs are reported. }
\begin{tabular}{cc|c|ccc|ccc|ccc|ccc}
\hline
\multicolumn{2}{c|}{Method} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Error\\ rate\end{tabular}} &
  \multicolumn{3}{c|}{Tiny ImageNet} &
  \multicolumn{3}{c|}{LSUN} &
  \multicolumn{3}{c|}{Place365} &
  \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Average\\ (total 6)\end{tabular}} \\ \cline{1-2} \cline{4-15} 
\multicolumn{1}{c|}{Name} &
  Gamma &
   &
  \multicolumn{1}{c|}{AUC} &
  \multicolumn{1}{c|}{AP} &
  FPR &
  \multicolumn{1}{c|}{AUC} &
  \multicolumn{1}{c|}{AP} &
  FPR &
  \multicolumn{1}{c|}{AUC} &
  \multicolumn{1}{c|}{AP} &
  FPR &
  \multicolumn{1}{c|}{AUC} &
  \multicolumn{1}{c|}{AP} &
  FPR \\ \hline
\multicolumn{1}{c|}{EnergyOE} &
  0.00 &
  59.35 &
  \multicolumn{1}{c|}{70.78} &
  \multicolumn{1}{c|}{55.90} &
  74.43 &
  \multicolumn{1}{c|}{81.61} &
  \multicolumn{1}{c|}{69.16} &
  57.37 &
  \multicolumn{1}{c|}{79.12} &
  \multicolumn{1}{c|}{89.09} &
  61.96 &
  \multicolumn{1}{c|}{76.40} &
  \multicolumn{1}{c|}{72.24} &
  64.54 \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Balanced \\ EnergyOE\end{tabular}}} &
  0.10 &
  59.10 &
  \multicolumn{1}{c|}{70.89} &
  \multicolumn{1}{c|}{55.85} &
  74.23 &
  \multicolumn{1}{c|}{81.94} &
  \multicolumn{1}{c|}{69.37} &
  56.53 &
  \multicolumn{1}{c|}{79.42} &
  \multicolumn{1}{c|}{89.18} &
  60.93 &
  \multicolumn{1}{c|}{76.66} &
  \multicolumn{1}{c|}{72.29} &
  63.82 \\
\multicolumn{1}{c|}{} &
  0.25 &
  58.50 &
  \multicolumn{1}{c|}{71.10} &
  \multicolumn{1}{c|}{55.85} &
  74.12 &
  \multicolumn{1}{c|}{82.35} &
  \multicolumn{1}{c|}{69.55} &
  55.50 &
  \multicolumn{1}{c|}{79.86} &
  \multicolumn{1}{c|}{89.31} &
  59.54 &
  \multicolumn{1}{c|}{76.92} &
  \multicolumn{1}{c|}{72.18} &
  62.96 \\
\multicolumn{1}{c|}{} &
  0.50 &
  \textbf{58.36} &
  \multicolumn{1}{c|}{71.36} &
  \multicolumn{1}{c|}{56.15} &
  \textbf{73.81}  &
  \multicolumn{1}{c|}{83.25} &
  \multicolumn{1}{c|}{70.48} &
  52.87 &
  \multicolumn{1}{c|}{80.65} &
  \multicolumn{1}{c|}{89.65} &
  58.09 &
  \multicolumn{1}{c|}{77.35} &
  \multicolumn{1}{c|}{72.50} &
  61.78 \\
\multicolumn{1}{c|}{} &
  0.75 &
  58.95 &
  \multicolumn{1}{c|}{\textbf{71.42}} &
  \multicolumn{1}{c|}{56.52} &
  74.22 &
  \multicolumn{1}{c|}{\textbf{83.83}} &
  \multicolumn{1}{c|}{71.23} &
  \textbf{52.04}  &
  \multicolumn{1}{c|}{81.10} &
  \multicolumn{1}{c|}{89.94} &
  \textbf{57.52}  &
  \multicolumn{1}{c|}{77.75} &
  \multicolumn{1}{c|}{73.10} &
  \textbf{61.15} \\
\multicolumn{1}{c|}{} &
  1.00 &
  61.38 &
  \multicolumn{1}{c|}{71.41} &
  \multicolumn{1}{c|}{56.76} &
  75.08 &
  \multicolumn{1}{c|}{83.76} &
  \multicolumn{1}{c|}{\textbf{71.40} } &
  53.46 &
  \multicolumn{1}{c|}{\textbf{81.12}} &
  \multicolumn{1}{c|}{\textbf{90.09}} &
  58.79 &
  \multicolumn{1}{c|}{\textbf{78.01}} &
  \multicolumn{1}{c|}{73.70} &
  61.66 \\
\multicolumn{1}{c|}{} &
  1.25 &
  63.49 &
  \multicolumn{1}{c|}{71.38} &
  \multicolumn{1}{c|}{\textbf{56.81}} &
  75.18 &
  \multicolumn{1}{c|}{82.85} &
  \multicolumn{1}{c|}{70.92} &
  58.68 &
  \multicolumn{1}{c|}{80.17} &
  \multicolumn{1}{c|}{89.83} &
  64.16 &
  \multicolumn{1}{c|}{77.96} &
  \multicolumn{1}{c|}{\textbf{73.97}} &
  63.08 \\ \hline
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Inv-Balanced\\  EnergyOE\end{tabular}} &
  -0.75 &
  65.23 &
  \multicolumn{1}{c|}{69.27} &
  \multicolumn{1}{c|}{55.59} &
  77.09 &
  \multicolumn{1}{c|}{80.20} &
  \multicolumn{1}{c|}{68.79} &
  66.63 &
  \multicolumn{1}{c|}{77.09} &
  \multicolumn{1}{c|}{88.64} &
  70.64 &
  \multicolumn{1}{c|}{75.14} &
  \multicolumn{1}{c|}{72.56} &
  70.71 \\ \hline
\end{tabular}
\end{table*}

==> cls_cifar100_validation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\small

\begin{tabular}{c|c|c|c|c}
\hline
Dataset                    & Method          & AUC            & AP             & FPR            \\ \hline
\multirow{5}{*}{Texture}   & OE (scratch)    & 76.71          & 58.79          & 68.28          \\
                           & PASCL           & 76.01          & 58.12          & 67.53          \\
                           & OE (tune)       & 66.29          & 51.98          & 84.04          \\
                           & EnergyOE (tune) & 79.56          & 70.88          & 68.60          \\ \cline{2-5} 
                           & Ours            & \textbf{82.10} & \textbf{73.09} & \textbf{64.19} \\ \hline
\multirow{5}{*}{SVHN}      & OE (scratch)    & 77.61          & 86.82          & 58.04          \\
                           & PASCL           & 80.19          & 88.49          & 53.45          \\
                           & OE (tune)       & 74.93          & 85.41          & 63.94          \\
                           & EnergyOE (tune) & 86.19          & 91.74          & 42.27          \\ \cline{2-5} 
                           & Ours            & \textbf{88.66} & \textbf{92.88} & \textbf{33.79} \\ \hline
\multirow{5}{*}{CIFAR10}                                                 & OE (scratch) & 62.23 & \textbf{57.57} & 80.64 \\
                           & PASCL           & \textbf{62.33} & 57.14          & \textbf{79.55} \\
                           & OE (tune)       & 59.44          & 56.34          & 84.70          \\
                           & EnergyOE (tune) & 61.15          & 56.66          & 82.60          \\ \cline{2-5} 
                           & Ours            & 59.40          & 54.97          & 85.16          \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Tiny\\ ImageNet\end{tabular}} & OE (scratch) & 68.04 & 51.66          & 76.66 \\
                           & PASCL           & 68.20          & 51.53          & 76.11          \\
                           & OE (tune)       & 66.24          & 51.07          & 80.04          \\
                           & EnergyOE (tune) & 70.78          & 55.90          & 74.43          \\ \cline{2-5} 
                           & Ours            & \textbf{71.42} & \textbf{56.52} & \textbf{74.22} \\ \hline
\multirow{5}{*}{LSUN}      & OE (scratch)    & 77.10          & 61.42          & 63.98          \\
                           & PASCL           & 77.19          & 61.27          & 63.31          \\
                           & OE (tune)       & 73.46          & 59.07          & 73.05          \\
                           & EnergyOE (tune) & 81.61          & 69.16          & 57.37          \\ \cline{2-5} 
                           & Ours            & \textbf{83.83} & \textbf{71.23} & \textbf{52.04} \\ \hline
\multirow{5}{*}{Places365} & OE (scratch)    & 75.80          & 86.68          & 65.72          \\
                           & PASCL           & 76.02          & 86.52          & 64.81          \\
                           & OE (tune)       & 71.70          & 85.08          & 74.62          \\
                           & EnergyOE (tune) & 79.12          & 89.09          & 61.96          \\ \cline{2-5} 
                           & Ours            & \textbf{81.10} & \textbf{89.94} & \textbf{57.52} \\ \hline
\multirow{5}{*}{Average}   & OE (scratch)    & 72.91          & 67.16          & 68.89          \\
                           & PASCL           & 73.32          & 67.18          & 67.44          \\
                           & OE (tune)       & 68.68          & 64.83          & 76.73          \\
                           & EnergyOE (tune) & 76.40          & 72.24          & 64.54          \\ \cline{2-5} 
                           & Ours            & \textbf{77.75} & \textbf{73.10} & \textbf{61.15} \\ \hline
\end{tabular}
\end{table}

==> cls_cifar100_validation_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\scriptsize
\captionsetup{font=footnotesize}
\caption{Comparison result with other methods on CIFAR100-LT using ResNet18 : average (over 6 datasets) OOD detection performance (AUROC,AP, FPR) and classification accuracy (ACC)}
\label{table_cifar100_LT_summary}
\begin{tabular}{c|c|c|c|c|c}
\hline
Dataset                  & Method             & AUC            & AP             & FPR            & ACC            \\ \hline
\multirow{9}{*}{Average} & MSP~\cite{hendrycks2016baseline}(ST)           & 60.26          & 57.58          & 84.00          & 38.74          \\
                         & Energy~\cite{liu2020energy}(ST)        & 63.22          & 59.06          & 81.12          & 38.74          \\
                         & OECC~\cite{papadopoulos2021outlier}               & 70.38          & 66.87          & 73.15          & 32.93          \\
                         & EnergyOE~\cite{liu2020energy}(scratch) & 71.10          & 67.23          & 71.78          & 39.05          \\
                         & OE~\cite{hendrycks2018deep}(scratch)       & 72.91          & 67.16          & 68.89          & 39.04          \\
                         & PASCL~\cite{wang2022partial}             & 73.32          & 67.18          & 67.44          & \textbf{43.10} \\
                         & OE~\cite{hendrycks2018deep}(tune)          & 68.68          & 64.83          & 76.73          & 38.93          \\
                         & EnergyOE~\cite{liu2020energy}(tune)    & 76.40          & 72.24          & 64.54          & 40.65          \\ \cline{2-6} 
                         &  \textbf{Ours}               & \textbf{77.75} & \textbf{73.10} & \textbf{61.15} & 41.05          \\ \hline
\end{tabular}
\end{table}

==> cls_cifar100_validation_light.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\scriptsize
\captionsetup{font=footnotesize}
\caption{Evaluation result on CIFAR100-LT using ResNet18 : OOD detection performance with AUROC,AP and FPR; Mean over six random runs are reported(OE,EnergyOE,Ours).}
\label{table_cifar100_LT_all}
\begin{tabular}{c|c|c|c|c}
\hline
Dataset                    & Method          & AUC            & AP             & FPR            \\ \hline
\multirow{3}{*}{Texture}   & OE (tune)       & 66.29          & 51.98          & 84.04          \\
                           & EnergyOE (tune) & 79.56          & 70.88          & 68.60          \\ \cline{2-5} 
                           & \textbf{Ours}             & \textbf{82.10} & \textbf{73.09} & \textbf{64.19} \\ \hline
\multirow{3}{*}{SVHN}      & OE (tune)       & 74.93          & 85.41          & 63.94          \\
                           & EnergyOE (tune) & 86.19          & 91.74          & 42.27          \\ \cline{2-5} 
                           & \textbf{Ours}             & \textbf{88.66} & \textbf{92.88} & \textbf{33.79} \\ \hline
\multirow{3}{*}{CIFAR10}   & OE (tune)       & 59.44          & 56.34          & 84.70          \\
                                                                         & EnergyOE (tune) & \textbf{61.15} & \textbf{56.66} & \textbf{82.60} \\ \cline{2-5} 
                           & \textbf{Ours}             & 59.40          & 54.97          & 85.16          \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Tiny\\ ImageNet\end{tabular}} & OE (tune)       & 66.24          & 51.07          & 80.04          \\
                           & EnergyOE (tune) & 70.78          & 55.90          & 74.43          \\ \cline{2-5} 
                           & \textbf{Ours}             & \textbf{71.42} & \textbf{56.52} & \textbf{74.22} \\ \hline
\multirow{3}{*}{LSUN}      & OE (tune)       & 73.46          & 59.07          & 73.05          \\
                           & EnergyOE (tune) & 81.61          & 69.16          & 57.37          \\ \cline{2-5} 
                           & \textbf{Ours}             & \textbf{83.83} & \textbf{71.23} & \textbf{52.04} \\ \hline
\multirow{3}{*}{Places365} & OE (tune)       & 71.70          & 85.08          & 74.62          \\
                           & EnergyOE (tune) & 79.12          & 89.09          & 61.96          \\ \cline{2-5} 
                           & \textbf{Ours}             & \textbf{81.10} & \textbf{89.94} & \textbf{57.52} \\ \hline
\multirow{3}{*}{Average}   & OE (tune)       & 68.68          & 64.83          & 76.73          \\
                           & EnergyOE (tune) & 76.40          & 72.24          & 64.54          \\ \cline{2-5} 
                           & \textbf{Ours}            & \textbf{77.75} & \textbf{73.10} & \textbf{61.15} \\ \hline
\end{tabular}
\end{table}

==> cls_cifar100_wideres_gamma_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\centering
\footnotesize
\caption{Evaluation result on CIFAR100-LT in long-tailed image classification task depending on hyperparameter $\gamma$: OOD detection performance(AUROC,AP,FPR)
and accuracy(ACC) with model WideResNet(WRN-40-2); Mean over six random runs are reported.}
\begin{tabular}{cc|c|ccc|ccc|ccc|ccc}
\hline
\multicolumn{2}{c|}{Method} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Error\\ rate\end{tabular}} &
  \multicolumn{3}{c|}{Tiny ImageNet} &
  \multicolumn{3}{c|}{LSUN} &
  \multicolumn{3}{c|}{Place365} &
  \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Average\\ (total 6)\end{tabular}} \\ \cline{1-2} \cline{4-15} 
\multicolumn{1}{c|}{Name} &
  Gamma &
   &
  \multicolumn{1}{c|}{AUC} &
  \multicolumn{1}{c|}{AP} &
  FPR &
  \multicolumn{1}{c|}{AUC} &
  \multicolumn{1}{c|}{AP} &
  FPR &
  \multicolumn{1}{c|}{AUC} &
  \multicolumn{1}{c|}{AP} &
  FPR &
  \multicolumn{1}{c|}{AUC} &
  \multicolumn{1}{c|}{AP} &
  FPR \\ \hline
\multicolumn{1}{c|}{EnergyOE} &
  0.00 &
  60.05 &
  \multicolumn{1}{c|}{70.32} &
  \multicolumn{1}{c|}{\textbf{56.65}} &
  77.08 &
  \multicolumn{1}{c|}{80.95} &
  \multicolumn{1}{c|}{69.93} &
  61.56 &
  \multicolumn{1}{c|}{79.95} &
  \multicolumn{1}{c|}{89.83} &
  61.62 &
  \multicolumn{1}{c|}{76.45} &
  \multicolumn{1}{c|}{72.75} &
  65.70 \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Balanced \\ EnergyOE\end{tabular}}} &
  0.10 &
  59.70 &
  \multicolumn{1}{c|}{70.40} &
  \multicolumn{1}{c|}{56.49} &
  76.79 &
  \multicolumn{1}{c|}{81.53} &
  \multicolumn{1}{c|}{70.21} &
  59.55 &
  \multicolumn{1}{c|}{80.36} &
  \multicolumn{1}{c|}{89.99} &
  60.28 &
  \multicolumn{1}{c|}{76.72} &
  \multicolumn{1}{c|}{72.70} &
  64.66 \\
\multicolumn{1}{c|}{} &
  0.25 &
  \textbf{59.57} &
  \multicolumn{1}{c|}{70.44} &
  \multicolumn{1}{c|}{56.15} &
  76.60 &
  \multicolumn{1}{c|}{82.29} &
  \multicolumn{1}{c|}{70.54} &
  56.84 &
  \multicolumn{1}{c|}{80.84} &
  \multicolumn{1}{c|}{90.17} &
  59.00 &
  \multicolumn{1}{c|}{77.03} &
  \multicolumn{1}{c|}{72.76} &
  63.61 \\
\multicolumn{1}{c|}{} &
  0.50 &
  60.56 &
  \multicolumn{1}{c|}{70.46} &
  \multicolumn{1}{c|}{56.07} &
  76.66 &
  \multicolumn{1}{c|}{\textbf{83.44}} &
  \multicolumn{1}{c|}{71.42} &
  \textbf{53.31}  &
  \multicolumn{1}{c|}{\textbf{81.45} } &
  \multicolumn{1}{c|}{\textbf{90.36}} &
  \textbf{57.25} &
  \multicolumn{1}{c|}{77.41} &
  \multicolumn{1}{c|}{73.10} &
  \textbf{62.84} \\
\multicolumn{1}{c|}{} &
  0.75 &
  64.40 &
  \multicolumn{1}{c|}{\textbf{70.59} } &
  \multicolumn{1}{c|}{56.41} &
  76.97 &
  \multicolumn{1}{c|}{83.42} &
  \multicolumn{1}{c|}{\textbf{71.63}} &
  54.27 &
  \multicolumn{1}{c|}{80.90} &
  \multicolumn{1}{c|}{90.20} &
  60.85 &
  \multicolumn{1}{c|}{\textbf{77.58}} &
  \multicolumn{1}{c|}{\textbf{73.52}} &
  63.44 \\
\multicolumn{1}{c|}{} &
  1.00 &
  67.55 &
  \multicolumn{1}{c|}{70.47} &
  \multicolumn{1}{c|}{56.46} &
  77.02 &
  \multicolumn{1}{c|}{80.78} &
  \multicolumn{1}{c|}{69.44} &
  65.38 &
  \multicolumn{1}{c|}{78.77} &
  \multicolumn{1}{c|}{89.36} &
  67.34 &
  \multicolumn{1}{c|}{76.97} &
  \multicolumn{1}{c|}{73.40} &
  66.17 \\
\multicolumn{1}{c|}{} &
  1.25 &
  69.62 &
  \multicolumn{1}{c|}{70.24} &
  \multicolumn{1}{c|}{56.41} &
  \textbf{76.32} &
  \multicolumn{1}{c|}{79.00} &
  \multicolumn{1}{c|}{67.9} &
  69.88 &
  \multicolumn{1}{c|}{77.10} &
  \multicolumn{1}{c|}{88.72} &
  70.86 &
  \multicolumn{1}{c|}{76.41} &
  \multicolumn{1}{c|}{73.25} &
  67.51 \\ \hline
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Inv-Balanced\\  EnergyOE\end{tabular}} &
  -0.75 &
  N/A &
  \multicolumn{1}{c|}{N/A} &
  \multicolumn{1}{c|}{N/A} &
  N/A &
  \multicolumn{1}{c|}{N/A} &
  \multicolumn{1}{c|}{N/A} &
  N/A &
  \multicolumn{1}{c|}{N/A} &
  \multicolumn{1}{c|}{N/A} &
  N/A &
  \multicolumn{1}{c|}{N/A} &
  \multicolumn{1}{c|}{N/A} &
  N/A \\ \hline
\end{tabular}
\end{table*}

==> cls_cifar100_wideres_validation_comparison.tex <==
\begin{table}[h]
\centering
\scriptsize
\captionsetup{font=footnotesize}
\caption{Comparison result with other methods on CIFAR 100-LT using WideResNet(WRN-40-2) : average (over 6 datasets) OOD detection performance (AUROC,AP, FPR) and classification accuracy (ACC)}
\label{table_LT_cls100_Wide}
\begin{tabular}{c|c|c|c|c|c}
\hline
Dataset                  & Method          & AUC            & AP             & FPR            & ACC            \\ \hline
\multirow{5}{*}{Average} & MSP~\cite{hendrycks2016baseline}(ST)        & 60.24          & 57.22          & 83.52          & 40.96          \\
                         & Energy~\cite{liu2020energy}(ST)     & 63.31          & 59.44          & 81.95          & 40.96          \\
                         & OE~\cite{hendrycks2018deep}(tune)       & 68.52          & 65.18          & 76.88          & \textbf{41.73} \\
                         & EnergyOE~\cite{liu2020energy}(tune) & 76.45          & 72.75          & 65.70          & 39.95          \\ \cline{2-6} 
                         &  \textbf{Ours}            & \textbf{77.41} & \textbf{73.10} & \textbf{62.84} & 39.44          \\ \hline
\end{tabular}
\end{table}

==> cls_cifar10_balanced_validation_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\scriptsize
\captionsetup{font=footnotesize}
\caption{Comparison result with other methods on CIFAR10 using ResNet18 : average (over 6 datasets) OOD detection performance (AUROC,AP, FPR) and classification accuracy (ACC)}
\label{table_cifar10_summary}
\begin{tabular}{c|c|c|c|c|c}
\hline
Dataset                  & Method          & AUC            & AP             & FPR           & ACC            \\ \hline
\multirow{5}{*}{Average} & MSP~\cite{hendrycks2016baseline}(ST)         & 89.25          & 86.63          & 31.32         & 93.69          \\
                         & Energy~\cite{liu2020energy}(ST)      & 91.55          & 89.88          & 29.07         & 93.69          \\
                         & OE~\cite{hendrycks2018deep}(tune)       & 95.46          & 95.04          & 18.63         & 94.79          \\
                         & EnergyOE~\cite{liu2020energy}(tune) & 98.08          & 98.15          & 9.63          & \textbf{95.83} \\ \cline{2-6} 
                         &  \textbf{Ours}           & \textbf{98.15} & \textbf{98.21} & \textbf{9.27} & 95.77          \\ \hline
\end{tabular}
\end{table}

==> cls_cifar10_validation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\small
\begin{tabular}{c|c|c|c|c}
\hline
Dataset                    & Method          & AUC            & AP             & FPR            \\ \hline
\multirow{5}{*}{Texture}   & OE (scratch)    & 92.59          & 83.32          & 25.10          \\
                           & PASCL           & 93.16          & 84.80          & 23.26          \\
                           & OE (tune)       & 87.98          & 80.05          & 45.54          \\
                           & EnergyOE (tune) & 95.53          & \textbf{92.93} & 23.26          \\ \cline{2-5} 
                           & Ours            & \textbf{95.69} & 92.38          & \textbf{21.26} \\ \hline
\multirow{5}{*}{SVHN}      & OE (scratch)    & 95.10          & 97.14          & 16.15          \\
                           & PASCL           & 96.63          & 98.06          & 12.18          \\
                           & OE (tune)       & 92.10          & 95.52          & 27.37          \\
                           & EnergyOE (tune) & 96.63          & 98.46          & 14.52          \\ \cline{2-5} 
                           & Ours            & \textbf{97.74} & \textbf{98.89} & \textbf{9.87}  \\ \hline
\multirow{5}{*}{CIFAR100}                                                & OE (scratch) & 83.40 & 80.93 & \textbf{56.96} \\
                           & PASCL           & 84.43          & 82.99          & 57.27          \\
                           & OE (tune)       & 78.24          & 76.35          & 65.28          \\
                           & EnergyOE (tune) & 84.44          & 84.63          & 59.92          \\ \cline{2-5} 
                           & Ours            & \textbf{85.20} & \textbf{84.98} & 57.95          \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Tiny\\ ImageNet\end{tabular}} & OE (scratch) & 86.14 & 79.33 & 47.78          \\
                           & PASCL           & 87.14          & 81.54          & 47.69          \\
                           & OE (tune)       & 81.47          & 75.79          & 58.68          \\
                           & EnergyOE (tune) & 88.40          & 84.95          & 45.17          \\ \cline{2-5} 
                           & Ours            & \textbf{88.92} & \textbf{84.98} & \textbf{42.38} \\ \hline
\multirow{5}{*}{LSUN}      & OE (scratch)    & 91.35          & 87.62          & 27.86          \\
                           & PASCL           & 93.17          & 91.76          & 26.40          \\
                           & OE (tune)       & 86.19          & 85.85          & 54.49          \\
                           & EnergyOE (tune) & 94.00          & \textbf{93.70} & 26.96          \\ \cline{2-5} 
                           & Ours            & \textbf{94.48} & 93.15          & \textbf{23.88} \\ \hline
\multirow{5}{*}{Places365} & OE (scratch)    & 90.07          & 95.15          & 34.04          \\
                           & PASCL           & 91.43          & 96.28          & 33.40          \\
                           & OE (tune)       & 84.27          & 93.84          & 59.08          \\
                           & EnergyOE (tune) & 92.51          & 97.14          & 32.88          \\ \cline{2-5} 
                           & Ours            & \textbf{93.35} & \textbf{97.23} & \textbf{28.25} \\ \hline
\multirow{5}{*}{Average}   & OE (scratch)    & 89.77          & 87.25          & 34.65          \\
                           & PASCL           & 90.99          & 89.24          & 33.36          \\
                           & OE (tune)       & 85.04          & 84.57          & 51.74          \\
                           & EnergyOE (tune) & 91.92          & \textbf{91.97} & 33.79          \\ \cline{2-5} 
                           & Ours            & \textbf{92.56} & 91.94          & \textbf{30.60} \\ \hline
\end{tabular}
\end{table}

==> cls_cifar10_validation_comparison.tex <==
\begin{table}[h]
\centering
\scriptsize
\captionsetup{font=footnotesize}
\caption{Comparison result with other methods on CIFAR10-LT using ResNet18 : average (over 6 datasets) OOD detection performance (AUROC,AP, FPR) and classification accuracy (ACC)}
\label{table_cifar10_LT_summary}
\begin{tabular}{c|c|c|c|c|c}
\hline
Dataset                  & Method             & AUC            & AP             & FPR            & ACC            \\ \hline
\multirow{9}{*}{Average} & MSP~\cite{hendrycks2016baseline}(ST)           & 70.96          & 69.35          & 67.37          & 69.83          \\
                         & Energy~\cite{liu2020energy}(ST)        & 75.93          & 72.91          & 61.00          & 69.83          \\
                         & OECC~\cite{papadopoulos2021outlier}               & 87.28          & 86.29          & 45.24          & 60.16          \\
                         & EnergyOE~\cite{liu2020energy}(scratch) & 89.31          & 88.92          & 40.88          & 74.68          \\
                         & OE~\cite{hendrycks2018deep}(scratch)       & 89.77          & 87.25          & 34.65          & 73.84          \\
                         & PASCL~\cite{wang2022partial}             & 90.99          & 89.24          & 33.36          & \textbf{77.08} \\
                         & OE~\cite{hendrycks2018deep}(tune)          & 85.04          & 84.57          & 51.74          & 69.79          \\
                         & EnergyOE~\cite{liu2020energy}(tune)    & 91.92          & \textbf{91.97} & 33.79          & 74.53          \\ \cline{2-6} 
                         & \textbf{Ours}               & \textbf{92.56} & 91.94          & \textbf{30.60} & 76.22          \\ \hline
\end{tabular}
\end{table}

==> cls_cifar10_validation_light.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\scriptsize
\captionsetup{font=footnotesize}
\caption{Evaluation result on CIFAR10-LT using ResNet18 : OOD detection performance with AUROC,AP and FPR; Mean over six random runs are reported(OE,EnergyOE,Ours).}
\label{table_cifar10_LT_all}
\begin{tabular}{c|c|c|c|c}
\hline
Dataset                    & Method          & AUC            & AP             & FPR            \\ \hline
\multirow{3}{*}{Texture}   & OE (tune)       & 87.98          & 80.05          & 45.54          \\
                           & EnergyOE (tune) & 95.53          & \textbf{92.93} & 23.26          \\ \cline{2-5} 
                           & \textbf{Ours}            & \textbf{95.69} & 92.38          & \textbf{21.26} \\ \hline
\multirow{3}{*}{SVHN}      & OE (tune)       & 92.10          & 95.52          & 27.37          \\
                           & EnergyOE (tune) & 96.63          & 98.46          & 14.52          \\ \cline{2-5} 
                           & Ours            & \textbf{97.74} & \textbf{98.89} & \textbf{9.87}  \\ \hline
\multirow{3}{*}{CIFAR100}  & OE (tune)       & 78.24          & 76.35          & 65.28          \\
                           & EnergyOE (tune) & 84.44          & 84.63          & 59.92          \\ \cline{2-5} 
                           & \textbf{Ours}             & \textbf{85.20} & \textbf{84.98} & \textbf{57.95} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Tiny\\ ImageNet\end{tabular}} & OE (tune) & 81.47 & 75.79 & 58.68 \\
                           & EnergyOE (tune) & 88.40          & 84.95          & 45.17          \\ \cline{2-5} 
                           & \textbf{Ours}             & \textbf{88.92} & \textbf{84.98} & \textbf{42.38} \\ \hline
\multirow{3}{*}{LSUN}      & OE (tune)       & 86.19          & 85.85          & 54.49          \\
                           & EnergyOE (tune) & 94.00          & \textbf{93.70} & 26.96          \\ \cline{2-5} 
                           & \textbf{Ours}             & \textbf{94.48} & 93.15          & \textbf{23.88} \\ \hline
\multirow{3}{*}{Places365} & OE (tune)       & 84.27          & 93.84          & 59.08          \\
                           & EnergyOE (tune) & 92.51          & 97.14          & 32.88          \\ \cline{2-5} 
                           & \textbf{Ours}            & \textbf{93.35} & \textbf{97.23} & \textbf{28.25} \\ \hline
\multirow{3}{*}{Average}   & OE (tune)       & 85.04          & 84.57          & 51.74          \\
                           & EnergyOE (tune) & 91.92          & \textbf{91.97} & 33.79          \\ \cline{2-5} 
                           & \textbf{Ours}             & \textbf{92.56} & 91.94          & \textbf{30.60} \\ \hline
\end{tabular}
\end{table}

==> cls_cifar10_wideres_gamma_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\centering
\footnotesize
\caption{Evaluation result on CIFAR10-LT in long-tailed image classification task depending on hyperparameter $\gamma$: OOD detection performance(AUROC,AP,FPR)
and accuracy(ACC) with model WideResNet(WRN-40-2); Mean over six random runs are reported.}
\begin{tabular}{cc|c|ccc|ccc|ccc|ccc}
\hline
\multicolumn{2}{c|}{Method} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Error\\ rate\end{tabular}} &
  \multicolumn{3}{c|}{Tiny ImageNet} &
  \multicolumn{3}{c|}{LSUN} &
  \multicolumn{3}{c|}{Place365} &
  \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Average\\ (total 6)\end{tabular}} \\ \cline{1-2} \cline{4-15} 
\multicolumn{1}{c|}{Name} &
  Gamma &
   &
  \multicolumn{1}{c|}{AUC} &
  \multicolumn{1}{c|}{AP} &
  FPR &
  \multicolumn{1}{c|}{AUC} &
  \multicolumn{1}{c|}{AP} &
  FPR &
  \multicolumn{1}{c|}{AUC} &
  \multicolumn{1}{c|}{AP} &
  FPR &
  \multicolumn{1}{c|}{AUC} &
  \multicolumn{1}{c|}{AP} &
  FPR \\ \hline
\multicolumn{1}{c|}{EnergyOE} &
  0.00 &
  24.97 &
  \multicolumn{1}{c|}{87.63} &
  \multicolumn{1}{c|}{\textbf{83.86}} &
  47.77 &
  \multicolumn{1}{c|}{94.80} &
  \multicolumn{1}{c|}{\textbf{94.41}} &
  24.17 &
  \multicolumn{1}{c|}{92.72} &
  \multicolumn{1}{c|}{97.17} &
  31.58 &
  \multicolumn{1}{c|}{91.44} &
  \multicolumn{1}{c|}{91.01} &
  34.02 \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Balanced \\ EnergyOE\end{tabular}}} &
  0.10 &
  24.72 &
  \multicolumn{1}{c|}{87.82} &
  \multicolumn{1}{c|}{83.75} &
  46.80 &
  \multicolumn{1}{c|}{94.78} &
  \multicolumn{1}{c|}{93.81} &
  22.68 &
  \multicolumn{1}{c|}{92.84} &
  \multicolumn{1}{c|}{97.06} &
  29.98 &
  \multicolumn{1}{c|}{91.57} &
  \multicolumn{1}{c|}{90.67} &
  32.78 \\
\multicolumn{1}{c|}{} &
  0.25 &
  24.26 &
  \multicolumn{1}{c|}{87.97} &
  \multicolumn{1}{c|}{83.61} &
  45.47 &
  \multicolumn{1}{c|}{94.72} &
  \multicolumn{1}{c|}{93.03} &
  21.51 &
  \multicolumn{1}{c|}{92.89} &
  \multicolumn{1}{c|}{96.89} &
  28.90 &
  \multicolumn{1}{c|}{91.65} &
  \multicolumn{1}{c|}{90.34} &
  31.75 \\
\multicolumn{1}{c|}{} &
  0.50 &
  \textbf{23.86} &
  \multicolumn{1}{c|}{\textbf{88.12} } &
  \multicolumn{1}{c|}{\textbf{83.76} } &
  \textbf{44.61}  &
  \multicolumn{1}{c|}{94.90} &
  \multicolumn{1}{c|}{93.23} &
  \textbf{20.45}  &
  \multicolumn{1}{c|}{93.16} &
  \multicolumn{1}{c|}{96.96} &
  \textbf{27.61} &
  \multicolumn{1}{c|}{\textbf{91.85}} &
  \multicolumn{1}{c|}{90.48} &
  \textbf{31.03} \\
\multicolumn{1}{c|}{} &
  0.75 &
  25.24 &
  \multicolumn{1}{c|}{87.91} &
  \multicolumn{1}{c|}{83.71} &
  45.68 &
  \multicolumn{1}{c|}{\textbf{94.94}} &
  \multicolumn{1}{c|}{93.67} &
  20.91 &
  \multicolumn{1}{c|}{\textbf{93.19} } &
  \multicolumn{1}{c|}{97.05} &
  28.25 &
  \multicolumn{1}{c|}{91.83} &
  \multicolumn{1}{c|}{90.66} &
  31.69 \\
\multicolumn{1}{c|}{} &
  1.00 &
  28.80 &
  \multicolumn{1}{c|}{87.59} &
  \multicolumn{1}{c|}{83.56} &
  47.68 &
  \multicolumn{1}{c|}{94.91} &
  \multicolumn{1}{c|}{94.25} &
  22.63 &
  \multicolumn{1}{c|}{\textbf{93.19} } &
  \multicolumn{1}{c|}{97.21} &
  29.08 &
  \multicolumn{1}{c|}{91.72} &
  \multicolumn{1}{c|}{91.01} &
  33.29 \\
\multicolumn{1}{c|}{} &
  1.25 &
  31.30 &
  \multicolumn{1}{c|}{87.22} &
  \multicolumn{1}{c|}{83.42} &
  48.87 &
  \multicolumn{1}{c|}{94.81} &
  \multicolumn{1}{c|}{92.28} &
  23.16 &
  \multicolumn{1}{c|}{93.06} &
  \multicolumn{1}{c|}{\textbf{97.22}} &
  30.14 &
  \multicolumn{1}{c|}{91.56} &
  \multicolumn{1}{c|}{\textbf{91.11}} &
  34.46 \\ \hline
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Inv-Balanced\\  EnergyOE\end{tabular}} &
  -0.75 &
  37.09 &
  \multicolumn{1}{c|}{84.81} &
  \multicolumn{1}{c|}{81.26} &
  56.31 &
  \multicolumn{1}{c|}{92.93} &
  \multicolumn{1}{c|}{92.66} &
  36.62 &
  \multicolumn{1}{c|}{90.38} &
  \multicolumn{1}{c|}{96.35} &
  44.05 &
  \multicolumn{1}{c|}{89.34} &
  \multicolumn{1}{c|}{89.81} &
  44.41 \\ \hline
\end{tabular}
\end{table*}

==> cls_cifar10_wideres_validation_comparison.tex <==
\begin{table}[h]
\centering
\scriptsize
\captionsetup{font=footnotesize}
\caption{Comparison result with other methods on CIFAR10-LT using WideResNet(WRN-40-2) : average (over 6 datasets) OOD detection performance (AUROC,AP, FPR) and classification accuracy (ACC)}
\label{table_LT_cls10_Wide}
\begin{tabular}{c|c|c|c|c|c}
\hline
Dataset                  & Method          & AUC            & AP             & FPR            & ACC            \\ \hline
\multirow{5}{*}{Average} & MSP~\cite{hendrycks2016baseline}(ST)        & 74.59          & 72.62          & 63.96          & 72.32          \\
                         & Energy~\cite{liu2020energy}(ST)     & 80.23          & 77.67          & 58.44          & 72.32          \\
                         & OE~\cite{hendrycks2018deep}(tune)       & 83.96          & 83.70          & 54.60          & 69.31          \\
                         & EnergyOE~\cite{liu2020energy}(tune) & 91.44          & \textbf{91.01} & 34.02          & 75.02          \\ \cline{2-6} 
                         &  \textbf{Ours}            & \textbf{91.85} & 90.48          & \textbf{31.03} & \textbf{76.14} \\ \hline
\end{tabular}
\end{table}

==> cls_element_balanced_ablation.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%
% 크게 의미가 없어서 뺴도 될것같은느낌
%
%%%%%%%%%%


\begin{table}[h]
\centering
\footnotesize
{Ablation results of loss component on both CIFAR10 and CIFAR100(image classification)
}
\begin{tabular}{cc|ccc|ccc}
\hline
\multicolumn{2}{c|}{Loss Component} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}CIFAR10-LT\\ Average\end{tabular}} &
  \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}CIFAR100-LT\\ Average\end{tabular}} \\ \hline
Margin & Weight & \multicolumn{1}{c|}{AUC}   & \multicolumn{1}{c|}{AP}    & FPR  & \multicolumn{1}{c|}{AUC}   & \multicolumn{1}{c|}{AP}    & FPR   \\ \hline
X      & X        & \multicolumn{1}{c|}{98.14} & \multicolumn{1}{c|}{98.18} & 9.31 & \multicolumn{1}{c|}{91.42} & \multicolumn{1}{c|}{88.30} & 33.29 \\
X      & O        & \multicolumn{1}{c|}{98.08} & \multicolumn{1}{c|}{98.15} & 9.59 & \multicolumn{1}{c|}{91.42} & \multicolumn{1}{c|}{88.29} & 33.28 \\
O &
  X &
  \multicolumn{1}{c|}{98.14} &
  \multicolumn{1}{c|}{\textbf{98.21}} &
  9.28 &
  \multicolumn{1}{c|}{\textbf{91.54}} &
  \multicolumn{1}{c|}{\textbf{88.33}} &
  32.66 \\
O &
  O &
  \multicolumn{1}{c|}{\textbf{98.15}} &
  \multicolumn{1}{c|}{\textbf{98.21}} &
  \textbf{9.27} &
  \multicolumn{1}{c|}{91.53} &
  \multicolumn{1}{c|}{88.32} &
  \textbf{32.65} \\ \hline
\end{tabular}
\end{table}
